Ranking Policy Decisions

Policies trained via Reinforcement Learning (RL) are often needlessly complex, making them difficult to analyse and interpret. In a run with $n$ time steps, a policy will make $n$ decisions on actions to take; we conjecture that only a small subset of these decisions delivers value over selecting a simple default action. Given a trained policy, we propose a novel black-box method based on statistical fault localisation that ranks the states of the environment according to the importance of decisions made in those states. We argue that among other things, the ranked list of states can help explain and understand the policy. As the ranking method is statistical, a direct evaluation of its quality is hard. As a proxy for quality, we use the ranking to create new, simpler policies from the original ones by pruning decisions identified as unimportant (that is, replacing them by default actions) and measuring the impact on performance. Our experiments on a diverse set of standard benchmarks demonstrate that pruned policies can perform on a level comparable to the original policies. Conversely, we show that naive approaches for ranking policy decisions, e.g., ranking based on the frequency of visiting a state, do not result in high-performing pruned policies.

==> Ranking Policy Decisions/approach.tex <==
\section{Method: ranking policy decisions using SBFL}\label{sec:approach}

Inspired by the use of SBFL for localising the cause of a program's outcome,
we propose a new SBFL-based method to identify the states in which 
decisions made by an RL policy are most important for achieving its
objective.
Our method is modular and is composed of two phases:
(1)~generating mutant policies and  (2)~ranking states based on the importance.
%and (3) constructing a pruned policy. 

\subsection{Definitions}\label{sec:def}

\paragraph{Executions of RL policies}

We apply the SBFL technique to a set of \emph{executions}
(sometimes called \emph{trajectories} in the literature) of a given RL policy $\pi$ with 
mutations. An \emph{execution} $\tau$ of $\pi$ describes a traversal of the agent through the environment MDP
using the RL policy~$\pi$ and is defined as a sequence of states $s_0, s_1, \ldots$ and actions $a_0, a_1, \ldots$,
where $s_0$ is an initial state and each subsequent state $s_{i+1}$ obtained from the previous state $s_i$ by performing
action~$a_i$, as chosen using $\pi(s_i)$. The last state must be a terminal state. As $\pi$ or the environment can be
stochastic, each execution of $\pi$ may result in a different sequence of actions and states, and hence in
a different $\tau$. The set of all possible executions is denoted by $\mathcal{T} $.
A \emph{decision} of a policy $\pi$ in a state $s$ is a pair $\langle s, \pi(s) \rangle$. Note that $\pi(s)$ is the learned probability distribution
from which an action in this state is obtained; in a deterministic policy, $\pi(s)$ is a single action for each $s$.

\paragraph{Passing and failing executions}

An execution is either successful or failed. We define the success of an execution as a (binary)
value of a given assertion on this execution. For example, the assertion can be that
the agent reaches its destination eventually, or that the reward of this execution is
not lower than $0.75$ of the maximal reward for $\pi$. The assertion induces a Boolean
function $C: \mathcal{T} \rightarrow \{0, 1\}$. We say that an execution~$\tau$ is a \emph{pass} if $C(\tau) = 1$, and is a
\emph{fail} otherwise. We use a binary condition for simplicity, as SBFL is 
designed to work with passing and failing executions. This condition 
can be relaxed \cite{DBLP:conf/ecai/CardosoAFK16}, and we plan to investigate 
generalising this in future work.

\paragraph{Mutant executions}

We use SBFL to understand the impact 
of replacing actions by a \emph{default action}.
The choice of the default action $d$ is context dependent and can
be configured by the user. For example, an obvious default
action for navigation is ``proceed in the same direction''.
The default action can in principle be as basic as a single action,
or as complex as a fully-fledged policy. In our experiments,
we evaluate two default actions. The first is ``repeat the previous action'', defined as:
%
\begin{equation}
d(s_0, \ldots, s_i, a_0, \ldots, a_{i-1}) = a_{i-1},
\end{equation}
%
and the second is ``take a random action''. For $A$ being the action space,
\begin{equation}
d(s_0, \ldots, s_i, a_0, \ldots, a_{i-1}) = a_{s_i} \sim \mathit{Unif}(A).
\end{equation}
%
Once $a_{s_i}$ has been sampled, it is not re-sampled if the state
$s_i$ is revisited; the same action is used.
Using ``take a random action'' as the default action can be useful in cases where there is no other obvious default action. 
However, we generally expect this to be a worse option than a default action tailored to the environment. As the choice of $d$ depends on the context and the user's goals, it is ultimately a user choice.

Using the default action, we create \emph{mutant executions},
in which the agent takes the default action $d$ whenever 
it is in one of the \emph{mutant states}. More formally, given a 
set of mutant states $S_M$, we act according to the policy $\pi_{S_M}$
defined as:
%
\begin{equation}\label{eq:lazypolicy}
\pi_{S_M}(s_0, \ldots, s_i, a_0, \ldots, a_{i-1}) = 
\begin{cases}
\pi(s_i) & s_i \notin S_M, \\ 
d(s_0, \ldots, s_i, a_0, \ldots, a_{i-1}) & s_i \in S_M.
\end{cases}
\end{equation}
%

Decisions made in states in which the default action is a very good option are deemed less important. 
In these states, not following the policy would be less consequential.

% \substituted{The choice of $d$ has a large influence on the results, as it is with respect to 
% this action that we determine the `importance' of the policy's decision.}
% {
% Though the choice of $d$ has a large influence on the results, as it is with respect to 
% this action that we determine the `importance' of the policy's decision, the decision ranking could be used to confirm if the default action is chosen properly (e.g., via evaluating performance of the pruned policy in Section \ref{sec:prunedpol}).
% }
% \ys{Please check}

\subsection{Generating the test suite and mutant executions on-the-fly}
\label{sec:testsuite}

The na\"ive approach to generating a comprehensive suite of mutant executions for applying SBFL would be to
consider all possible sets of mutant states $S_M$---that is, we would need to consider all possible subsets of the state space~$S$. 
% \added{that overlap with $S_M$}. \ys{Please check}
However, the state space of most RL environments is too large to enumerate, and enumerating all
possible subsets of $S$ is intractable even for simplistic environments.

We use two algorithmic techniques to address this problem: (a)~we generate
mutant executions \emph{on-the-fly}, and (b)~we use an abstraction function
$\alpha : S \rightarrow \hat S$ to map the full set of states $S$ to a smaller, less complex
set of abstract states $\hat S$. Examples of these are in the supplementary material,
and may for example include down-scaling or grey-scaling images that are input 
to the agent, or quantising a continuous state space. 
The set of possible mutations is then the set of subsets
of $\hat S$, instead of the set of subsets of~$S$. We then score the abstract states, rather than the full state space. The test suite of 
mutant executions produced 
this way for $\pi$ is denoted $\mathcal{T}(\pi) \subseteq \mathcal{T}$.

\paragraph{On-the-fly mutation}

We maintain a set $S_M \subseteq \hat S$ per execution. We begin each execution 
$\tau$ by initialising
the set $S_M$ with the empty set of states.
At each step of the execution, upon visiting a state~$s$, we check the current $S_M$.
If $\alpha(s) \not\in S_M$, we add $\alpha(s)$ to $S_M$ according to the predefined \emph{mutation rate}~$\mu$
(and take the default action); otherwise, we use $\pi$ to determine the action in
this state. In case we re-visit an (abstract) state, we maintain the previous decision of whether to
mutate state $s$ or not. This way, the states that are never visited in any of the
executions are never mutated; hence, we never consider ``useless mutations'' that mutate a state
that is never visited. We finish by marking $\tau$ as
pass or fail according to $C(\tau)$.
Note that a mutant execution may visit states not typically encountered
by~$\pi$, meaning that we are even able to rank states that are out of distribution. This is especially important when trying to 
understand how the policy behaves in parts of the environment it 
is unfamiliar with.

Overall, our algorithm has five (tunable) parameters: the size of the test suite~$|\mathcal{T}(\pi)|$,
the passing condition~$C$,
the default action~$d$, the mutation rate~$\mu$ and the abstraction function~$\alpha$.

SBFL benefits from a balanced test suite of passing and failing 
executions~\cite{wong2016survey}, a ratio largely determined
by the choices of $\mu$ and $C$. The choice of $C$ depends on the context.
In our experiments in Section~\ref{sec:prunedpol}, 
our goal was to find the states with highest
impact on the expected reward. We set the condition to be ``receive more than $X$ 
reward" for some $X \in \mathbb{R}$, and chose $X$ to yield a balanced 
suite (i.e. if there were too many failed runs, we lowered $X$). 
% \ys{chose $X$ to produce a balanced test? Do not understand}
In most cases actions important for achieving at least $X$ reward
are important for maximising reward in general, so
we found that this worked well. In the cases where some actions 
are not important for achieving $X$, but later important for 
getting even higher rewards 
(e.g., states that only appear after achieving $X$ reward), 
we would not have considered them important. 
The choice of $\mu$ is also significant. If it is too large, executions
fail too often, and the behaviour in mutant executions is uninteresting.
If $\mu$ is too small, we do not mutate states
enough to learn anything, and in larger 
environments fail to mutate many of the states we encounter. 
In our experiments, we selected $\mu$ manually, but this could easily 
be automated by a parameter tuning algorithm.

\subsection{Computing the ranking of the policy decisions} %and constructing pruned policies}
\label{sec:rankings}%\label{sec:lazy}

We now explain how to rank states according to the importance of policy decisions made 
in these states, with respect to satisfying the condition.
The ranking method is based on SBFL as described in Section~\ref{sec:SFL}.
We first create the test suite of mutant 
executions $\mathcal{T}(\pi)$ as described above.
We denote the set of all abstract states encountered when generating the test suite $S_{\mathcal{T}} \subseteq \hat S$; these are the states to which we 
assign scores. Any unvisited state is given the lowest possible score by default.

Similarly to SBFL for bug localisation, for each state $s\in S_{\mathcal{T}}$ we
calculate a vector $\langle a^s_\mathit{ep}, a^s_\mathit{ef}, a^s_\mathit{np}, 
a^s_\mathit{nf} \rangle$. We use this vector to track 
the number of times that $s$ was unmutated ($e$) or mutated ($n$)
on passing ($p$) and on failing ($f$) executions, and
we update these scores based on those executions in which the state was visited.
In other words, the vector keeps track of
success and failure of mutant executions based on whether an execution took the 
default action in $s$ or not.
For example, $a^s_{ep}$ is the number of passing executions that took the action $\pi(s)$ 
in the state $s$, and $a^s_{nf}$ is the number of failing executions that took the default action
in the state~$s$. 
\begin{definition}[Ranking]\label{def-rank}
Given an SBFL measure $m$ and a vector
$\langle a^s_\mathit{ep}, a^s_\mathit{ef}, a^s_\mathit{np}, a^s_\mathit{nf} \rangle$ for each (abstract)
state $s$ in the set $\hat S$ of (abstract) states of the policy, we define the ranking function 
$\mathit{rank}: \hat S \rightarrow \{1,\ldots,|\hat S|\}$ as the ordering of the states in $\hat S$
in the descending order according to the values $m(s)$; that is, the state with the maximal value will be
the first in the ranking. 
%Once we have constructed the vector $\langle a^s_\mathit{ep}, a^s_\mathit{ef}, a^s_\mathit{np}, a^s_\mathit{nf} \rangle$
%for every (abstract) state, we apply the SBFL measures discussed in Section~\ref{sec:SFL} to rank the states in $\pi$.
%This ranking is denoted by $\mathit{rank}: \hat S \rightarrow \{1,\ldots,|\hat S|\}$.
\end{definition}

%For a state $s$ we compute the vector
%$\langle a^s_\mathit{ep}, a^s_\mathit{ef}, a^s_\mathit{np}, a^s_\mathit{nf} \rangle$ as follows:
%\begin{itemize}
%    \item $a^s_\mathit{ep}$ stands for the number of passing mutants $\tau$ in $\mathcal{T}(\pi)$ where ${\tau}(s) = \pi(s)$;
%    \item $a^s_\mathit{ef}$ stands for the number of failing mutants $\tau$ in $\mathcal{T}(\pi)$ where ${\tau}(s) = \pi(s)$;
%    \item $a^s_\mathit{np}$ stands for the number of passing mutants $\tau$ in $\mathcal{T}(\pi)$ where ${\tau}(s) = a_l$;
%    \item $a^s_\mathit{nf}$ stands for the number of failing mutants $\tau$ in $\mathcal{T}(\pi)$ where ${\tau}(s) = a_l$.
%\end{itemize}

==> Ranking Policy Decisions/background.tex <==
\section{Background}
\label{sec:background}

\subsection{Reinforcement learning (RL)}\label{sec:rl}

We use a standard reinforcement learning (RL) setup and assume that the reader is familiar with the basic concepts.
An \emph{environment} in RL is defined as a Markov decision process (MDP) and is 
denoted by $\langle S, A, P, R, \gamma, T\rangle$, where $S$ is the set of states, $A$ is the set of actions, $P$ is the transition function, $R$ is the reward function, $\gamma$ is the discount factor, and $T$ is the set of terminal states. An agent seeks to learn
a policy $\pi:S\rightarrow A$ that maximizes the total discounted reward. Starting from the initial state $s_0$ and given the policy $\pi$, the state-value function is the expected future discounted reward as follows:
%
\begin{equation}\label{eq:rlvalue}
V_{\pi}(s_0) = \mathbb{E}\left(\sum_{t=0}^{\infty}\gamma^tR(s_t,\pi(s_t),s_{t+1})\right)
\end{equation}
%
A policy $\pi: S \rightarrow A$ maps states to the actions taken in these states and may be  stochastic. We treat the policy as a black box, and hence make no further assumptions about $\pi$. 

\subsection{Spectrum-based fault localization (SBFL)}
\label{sec:SFL}

The reader is likely less familiar with spectrum-based fault localization (SBFL), as to the best
of our knowledge, it has not yet been used in RL. We therefore give a detailed description.
SBFL techniques~\cite{wong2016survey}
have been widely used as an efficient approach to aid in locating the
causes of failures in sequential programs. 
SBFL techniques rank program elements (say program statements)
based on their \emph{suspiciousness scores}, which are computed using correlation-based
measures. Intuitively, a program element is more suspicious if it appears in failed
executions more frequently than in correct executions, and the exact formulas differ between
the measures. Diagnosis of the faulty program can then be conducted by
manually examining the ranked list of elements
in descending order of their suspiciousness until the cause of the fault is found. It has
been shown that SBFL techniques perform well in complex programs \cite{abreu2009practical}.

SBFL techniques first execute the program under test using a \emph{test suite}.
A test suite comprises of a set of inputs and an expected output for each input. A test \emph{passes} when the output produced by the program under test matches the expected output given by the test suite, and has \emph{failed} otherwise.
In addition to the outcome of the test, SBFL techniques record the values of a set of Boolean flags that indicate whether a particular program element was executed by that test. 

The task of a fault localization tool is to compute a ranking of the program elements
based on the values of the Boolean flags recorded while executing the test suite.
Following the notation from~\cite{naish2011model}, the suspiciousness score of each
program statement $s$ is calculated from a set of parameters
$\langle a^s_\mathit{ep}, a^s_\mathit{ef}, a^s_\mathit{np}, a^s_\mathit{nf} \rangle$ that
give the number of times the statement $s$ is executed ($e$) or not executed~($n$) on passing ($p$)
and on failing ($f$) tests. For instance, $a^s_\mathit{ep}$ is the number of tests that passed and executed $s$.

Many measures have been proposed to calculate the suspicious scores of program elements.
In Equations~(\ref{eq:measures}a)$\sim$(\ref{eq:measures}d) we list a selection of popular and high-performing 
measures~\cite{abreu2007accuracy,zoltar,jones2005empirical,wong2007effective};
these are also the measures that we use in our ranking procedure.

\begin{subequations}\label{eq:measures}%
\begin{tabular}{@{\hspace{-0.2cm}}l@{}l}%
\begin{minipage}{6.5cm}%
\begin{equation}\text{Ochiai:}\,\,\, \frac{a_\mathit{ef}^s}{\sqrt{(a_\mathit{ef}^s+a_\mathit{nf}^s)(a_\mathit{ef}^s+a_\mathit{ep}^s)}}\label{eq:ochiai}\end{equation}
\end{minipage}
%
& \begin{minipage}{6.5cm}%
\begin{equation}
\hspace{1.2cm}\text{Tarantula:}\,\,\,  \displaystyle\frac{\frac{a_\mathit{ef}^s}{a_\mathit{ef}^s+a_\mathit{nf}^s}}{\frac{a_\mathit{ef}^s}{a_\mathit{ef}^s+a_\mathit{nf}^s}+\frac{a_\mathit{ep}^s}{a_\mathit{ep}^s+a_\mathit{np}^s}}\label{eq:tarantula}\end{equation}
\end{minipage}\\
%
\begin{minipage}{6.5cm}%
\begin{equation}\text{Zoltar:}\,\,\, \frac{a_\mathit{ef}^s}{a_\mathit{ef}^s+a_\mathit{nf}^s+a_\mathit{ep}^s+\frac{10000a_\mathit{nf}^sa_\mathit{ep}^s}{a_\mathit{ef}^{s}}}\end{equation}
\end{minipage}
%
& \begin{minipage}{6.5cm}%
\begin{equation}
\text{Wong-II:} \label{eq:wong-ii}\,\,\,   a_\mathit{ef}^s-a_\mathit{ep}^s
\end{equation}
\end{minipage}
\end{tabular}
\end{subequations}

\commentout{
\begin{subequations}\label{eq:measures}%
    \begin{equation}\text{Ochiai:}\,\,\, \frac{a_\mathit{ef}^s}{\sqrt{(a_\mathit{ef}^s+a_\mathit{nf}^s)(a_\mathit{ef}^s+a_\mathit{ep}^s)}}\label{eq:ochiai}\end{equation}

    \begin{equation}\text{Tarantula:}\,\,\,  \displaystyle\frac{\frac{a_\mathit{ef}^s}{a_\mathit{ef}^s+a_\mathit{nf}^s}}{\frac{a_\mathit{ef}^s}{a_\mathit{ef}^s+a_\mathit{nf}^s}+\frac{a_\mathit{ep}^s}{a_\mathit{ep}^s+a_\mathit{np}^s}}\label{eq:tarantula}\end{equation}
    
    \begin{equation}\text{Zoltar:}\,\,\, \frac{a_\mathit{ef}^s}{a_\mathit{ef}^s+a_\mathit{nf}^s+a_\mathit{ep}^s+\frac{10000a_\mathit{nf}^sa_\mathit{ep}^s}{a_\mathit{ef}^{s}}}\end{equation}

    \begin{equation}
    \text{Wong-II:} \label{eq:wong-ii}\,\,\,   a_\mathit{ef}^s-a_\mathit{ep}^s
    \end{equation}
\end{subequations}
}


SBFL-based tools present the list of program elements in descending order of their suspiciousness scores to the user. There is no single best measure for fault localization; different measures perform better on different types of programs, and it is best practice to use multiple measures \cite{lucia2014extended}. In our experiments, we combine the 
four measures listed above for this very reason.

While more sophisticated versions of SBFL exist \cite{DBLP:conf/ijcai/AbreuZG09,DBLP:conf/ecai/CardosoAFK16}, in this work we prefer to stick to the simpler approach, which was sufficient for producing notable results.

%From a more formal perspective, the four quantities in Eq. \ref{ex:measures} can be seen as either probabilistic epistemic uncertainty or conditional probability, and using test cases can be seen as a statistical estimation of the quantities. A bound can be even possible to
%measure the possible loss of the estimation \cite{landsberg2018optimising}.


==> Ranking Policy Decisions/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Ranking Policy Decisions/conclusion.tex <==
\section{Conclusions}

We have applied SBFL-based ranking of states to
reinforcement learning and demonstrated that this ranking correlates
with the relative importance of states for the policy's performance.
The ranking can be used to explain RL policies, similarly to the way ranked
program locations are used to understand the causes of a bug.  
We evaluate the quality of our ranking by constructing simpler
pruned policies, where only the most important decisions are made
according to the policy, and the rest are default. Our experiments show that the performance of the pruned policies is comparable to the performance of the original policies,
thus supporting our claim that the SBFL-based ranking is accurate.
Moreover, the pruned policies may be preferable in many use-cases, as they are simpler.
Our approach can be scaled with the use of abstractions, as demonstrated
by the larger Atari environments. 

In the future, we hope to explore different applications 
of the ranking, new measures, more nuanced hyperparameter selection,
and relaxing the binary constraint over the assertion $C$.
We do not expect our work to have any negative societal impacts, as it only serves to improve our understanding of the policies we train; the main
concern is incorrectly increasing confidence in a policy.

%SBFL's statistical approach helps make the problem tractable, 
%even in some larger Atari environments.
%In the environments we test, our method determines that many of the states
%are unimportant, and actions taken in those states can be replaced by a default 
%action with little impact on performance. We exploit this fact to 
%make more intuitive visualisations of the behaviour of a policy by focusing 
%attention to important states. We further show that our method can 
%help understand the difference between policies 
%(e.g.~a high and a low-quality policy), by considering their behaviour 
%according to the ranking of a state.

%Highlighting important states can help with analysing 
%the policy in both quantitative and qualitative ways, by eliminating 
%the need to consider states in which decisions have little influence.
%This could benefit explainability methods, in which removing unnecessary
%complexity is crucial. The \emph{pruned} policies we 
%produced to evaluate the rankings could serve as a more explainable
%versions of the original policy, as they leave fewer decisions to the 
%original policy, replacing them with simple default actions.
%In environments in which it is expensive to compute the 
%original policy's decision
%(e.g.~energy consumption when using a large neural network,
%or the cost of a human in the loop), it may be cheaper 
%to use a pruned policy, which makes cheap default decisions most 
%of the time. Of course, this depends on how expensive it is 
%to determine whether or not the state was pruned. In this paper we have shown
%that our rankings are successful in identifying important 
%states, and we have given examples of applications of these rankings. 
%We are optimistic that our method could be a powerful tool in furthering 
%our understand of the policies and their behaviour.

%
%the use of SBFL for understanding how an RL agent makes decisions, i.e., localizing these 
%more influential decisions that contribute to a RL policy. 
%This is an important step towards explainable RL. 

%Another aspect of robustness, which we plan to investigate in the future, is robustness against perturbations of
%the environment. We conjecture that the pruned policies might be more robust in this respect as well, as they
%avoid the danger of overfitting to a particular environment. 

%In the future, we plan to investigate robustness of pruned policies against 
%perturbations happen to the training environment. Our conjecture is that lazy policies are often
%more robust, as they avoid the danger of overfitting to a particular environment. 


==> Ranking Policy Decisions/evaluation.tex <==
\section{Experimental evaluation}\label{sec:evaluation}

\subsection{Research Questions}

Our goal is to demonstrate the applicability of our ranking method to
a variety of standard environments and to provide evidence of the utility
of the generated ranking. 
We aim to answer the following research questions:
%
\begin{description}
\item[RQ1:] How can we measure the relative importance of decisions for achieving the reward? What is a good proxy for measuring this?
\item[RQ2:] Does the approach we present in this paper scale to large policies and complex environments?
% \item[RQ3:] Can we use the ranking to explain policy decisions?
% \item[RQ4:] Can the ranking procedure be used to determine when the policy has been sufficiently trained?
\end{description}

We answer these questions in Section~\ref{sec:prunedpol} by performing extensive experiments with 
various environments and policies. In Section~\ref{sec:discussion}, we discuss
possible applications of our ranking (including interpretability), and the effect 
of choosing a different default action.

\subsection{Experimental setup}\label{sec:setup}

We experimented in several environments. The first is \emph{Minigrid}~\cite{gym_minigrid}, 
a gridworld in which the agent operates 
with a cone of vision and can navigate many different grids,
making it more complex than a standard gridworld. In each step the agent can turn or move forward.
We also used \emph{CartPole}~\cite{DBLP:journals/corr/BrockmanCPSSTZ16}, the classic control problem 
with a continuous state-space. Finally, to test our ability to scale, we ran experiments with 
\emph{Atari games}~\cite{DBLP:journals/corr/BrockmanCPSSTZ16}.

We use policies that are trained using third-party code.
No state abstraction is applied to the gridworld environments (i.e., $\alpha$ is the identity).
The state abstraction function for the CartPole environment consists 
of rounding the components of the state vector between 0 and 2 decimal places, 
and then taking the absolute value. For 
the Atari games, as is typically done,
we crop the game's border, 
grey-scale, down-sample to $18\times14$, and lower 
the precision of pixel intensities
to make the enormous state space manageable. Note that these 
abstractions are not a contribution of ours, and were primarily chosen
for their simplicity. 
For our main experiments, we use ``repeat previous action''
as the default action. 

Examples of some environments, and important states found 
in them, are given in Figs.~\ref{fig:vis_1} and~\ref{fig:vis_2}.
Details about the state abstraction functions,
policy training, hyperparameters, etc., are provided in 
\ifArxiv{Appendix~\ref{sec:exp_setup}}.
% The code is available on GitHub\footnote{\url{https://github.com/AnonUser-532438/PolicyRankingAnon}}, 
% and further examples are provided on the anonymised
% website\footnote{\url{https://sites.google.com/view/ranking-policy-decisions/}}.

We define two further measures in addition to the SBFL ones 
in Eq.~(\ref{eq:measures}), for comparison. Eq.~(\ref{eq:freqVis}) 
measures how frequently the state was encountered in the test suite. 
Eq.~(\ref{eq:rand}) is a random ranking
of the states visited by the test suite. We use the FreqVis measure as a
baseline because we are not aware of any previous work with the same goals 
as ours for ranking policy decisions, and a na\"ive approach to determining importance may be simply 
looking at how frequently a state is visited.

\begin{subequations}\label{eq:measures_baseline}%
\begin{tabular}{@{\hspace{-0.2cm}}l@{}l}%
\begin{minipage}[b]{6.6cm}%
\centering
\begin{equation}\text{FreqVis:}\,\,\, a_\mathit{ep}^s+a_\mathit{ef}^s+a_\mathit{np}^s+a_\mathit{nf}^s
\label{eq:freqVis}
\end{equation}
\end{minipage}
%
& \begin{minipage}[b]{5.8cm}%
\centering
\begin{equation}\text{Rand:}\,\,\,  \sim\text{Unif}(0, 1)
\label{eq:rand}
\end{equation}
\end{minipage}
\end{tabular}
\end{subequations}

\subsection{Experimental results}
\label{sec:prunedpol}

\paragraph{Performance of pruned policies}
The precise ranking of decisions according to their importance for the reward is intractable for all 
but very simple policies. To answer {\bf RQ1}, in our experiments, we
use the performance of 
\emph{pruned policies} as a \emph{proxy} for the quality of the ranking computed by our algorithm.
In pruned policies, the default action is used in all but the top ranked states.
%As a proxy for the quality of the ranking computed by our algorithm we compute the performance of
%the \emph{pruned policies}---these are policies where some of the actions
%are replaced by the default actions. The decision of whether or not to use the default
%action in a given state is based on the rank of the state. 
For a given $r$ (a fraction or a percentage), we denote
by $\mathit{rank}[r]$ the subset of $r$ top-ranked states.
We denote by~$\pi^r$ the pruned policy obtained by \emph{pruning}
all but the top-$r$ ranked states. That is, an execution of~$\pi^r$ retains actions in the $r$ fraction
of the most important states from the original policy $\pi$ and replaces the rest
by default actions. The states that are in
$\mathit{rank}[r]$ are called the \emph{original states}.
We measure the performance of the pruned policies for increasing values of $r$ relative to
the performance of the original policy $\pi$.
%To evaluate the quality of our ranking method, 
%we measure how quickly we are able to recover the
%performance of the original policy~$\pi$
%as we reduce set of pruned states. We start with $r=0$,
%and evaluate the performance of $\pi^r$ 
%for increasing values of $r$. 

These results are given in first four columns of Tab.~\ref{tab:pruning},
and some are represented graphically in Figs.~\ref{fig:graphs}a,c.
In these, SBFL stands for the \emph{SBFL portfolio}, i.e.,
the combination of the four measures in Eq.~(\ref{eq:measures}), where
the best result is taken at each point. 
The results show that the pruned policies obtained using the SBFL ranking 
can achieve performance that is comparable to $\pi$
with less than $40\%$ of the original decisions (and in 
some cases the number is as low as $20\%$).
The performance of SBFL-based pruning 
is compared with random pruning in Eq.~(\ref{eq:rand}) and
FreqVis pruning in Eq.~(\ref{eq:freqVis}). At first glance, it seems that the FreqVis pruned policies perform well in Figs.~\ref{fig:graphs}a,c.
To better understand this, we show in the last two columns of Tab.~\ref{tab:pruning} and 
in Figs.~\ref{fig:graphs}b,d how performance evolves with the proportion 
of steps in which the original policy is used over the default policy (i.e.~not replaced by the default action).
As shown in Figs.~\ref{fig:2} and~\ref{fig:6}, FreqVis does much worse by 
this metric, because it yields a pruned policy that
prefers to use the original policy as often as possible.
%We note that from 
%The difference in freqVis' success illustrates the 
%difference between the two ways of reporting performance.
%By restoring common 
%states first, it quickly recovers the original policy's
%behaviour (Figure~\ref{fig:1}), but also stops taking any 
%default actions (Figure~\ref{fig:2}).

%and selected results are explained in more detail in
%Figure~\ref{fig:graphs}.
%We look at both how performance is recovered as 
%the percentage of unpruned states increases,
%and as the percentage of steps 
%in which the original policy is used increases
%(note that for the former, we always prune all of 
%the states not encountered in the test 
%suite, even at 100\%).
%These two ways of reporting performance
%differ when, for example, we rank highly
%states that are important if visited but rare. Even if 
%many of theses states are not pruned, 
%the policy would still more often take the default 
%action, despite fewer states being pruned overall.
%Results are given in Table~\ref{tab:pruning},
%and selected results are explained in more detail in
%Figure~\ref{fig:graphs}.
%The difference in freqVis' success illustrates the 
%difference between the two ways of reporting performance.
%By restoring common 
%states first, it quickly recovers the original policy's
%behaviour (Figure~\ref{fig:1}), but also stops taking any 
%default actions (Figure~\ref{fig:2}).

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=.8\linewidth]{new_imgs/cartpole/struct.png}
        \caption{CartPole States in Pruned Policy}
        \label{fig:1}
    \end{subfigure}%
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=.8\linewidth]{new_imgs/cartpole/behav.png}
        \caption{CartPole Actions Taken}
        \label{fig:2}
    \end{subfigure}

    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=.8\linewidth]{new_imgs/krull/struct.png}
        \caption{Krull States in Pruned Policy}
        \label{fig:5}%
    \end{subfigure}
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=.8\linewidth]{new_imgs/krull/behav.png}
        \caption{Krull Actions Taken}
        \label{fig:6}
    \end{subfigure}

    \caption{
    Performance of the pruned policies,
    measured as
    a percentage of the original reward.
%    Graphs show how quickly reducing set of pruned
%    states according to different measures
%    recovers performance.
 %   Y-axis is percentage of original reward,
 %   where 0\% is the reward of a random policy.
    \textbf{(a)},\textbf{(c)}: 
%    \textbf{Left Column:} 
    The $x$-axis is the \% of states where the original action is taken
    out of the set of all states encountered in the test suite.
%    restored, of the states that were 
%    encountered in the test suite.
    \textbf{(b)},\textbf{(d)}:
%    \textbf{Right column:} 
    The $x$-axis is the expected \%
    of steps in which the original policy is 
    followed over the default action during 
    an execution of the pruned policy. See the supplementary material for more detail.}
    \label{fig:graphs}
\end{figure}

\begin{table*}[t]
	\centering
    \caption{Minimum percentage of original states in pruned policies, and percentage
    of steps in which the original policy is used, before recovering 90\% 
    of original performance. Using default action ``repeat previous action''. Results are reported 
    for the SBFL portfolio ranking and the random ranking. ``\fail'' 
    denotes that the required reward was never reached,
    cf.~Sec.~\ref{sec:prunedpol}.
	}
	\label{tab:pruning}
% 	\small
	\newcolumntype{R}{>{\raggedleft\arraybackslash$}X<{$}}
	\newcolumntype{Y}{>{\centering\arraybackslash$}X<{$}}
	\begin{tabularx}{\linewidth}{@{}lYYYY}
		\toprule
        & \multicolumn{2}{c}{\% of original states restored} & \multicolumn{2}{c}{\% of steps that use $\pi$} \\ 
        %  & \multicolumn{2}{c}{For 90\% of orig. reward} & \multicolumn{2}{c}{For 90\% of orig. reward} \\
        \cmidrule{2-5}
        Environment & \mbox{SBFL} & \mbox{random} & \mbox{SBFL} & \mbox{random} \\
        \toprule
		MiniGrid & \mathbf{49} \pm 00  & 99 \pm 00 & \mathbf{76} \pm 00 & 98 \pm 01 \\
        \midrule
        Cartpole & \mathbf{31} \pm 04 & 65 \pm 02 & \mathbf{22} \pm 04 & 69 \pm 02 \\ 
        \midrule
        Alien & \fail & \fail & \fail & \fail \\
        Assault & \mathbf{45} \pm 07 & 100 \pm 00 & \mathbf{93} \pm 01 & 100 \pm 00 \\
        Atlantis & \mathbf{50} \pm 00 & 100 \pm 00 & \mathbf{99} \pm 00 & 100 \pm 00 \\
        BankHeist & \fail & \fail & \fail & \fail \\
        BattleZone & \mathbf{30} \pm 00 & 86 \pm 07 & \mathbf{84} \pm 07 & 84 \pm 08 \\
        Berzerk & \mathbf{47} \pm 12 & 100 \pm 00 & \mathbf{88} \pm 03 & 100 \pm 00 \\
        Boxing & \fail & \fail & \fail & \fail \\
        Breakout & \mathbf{10} \pm 00 & 100 \pm 00 & \mathbf{54} \pm 00 & 99 \pm 01 \\
        Breakout (abs) & \mathbf{40} \pm 00 & 85 \pm 05 & \mathbf{41} \pm 00 & 81 \pm 06 \\
        ChpperCmmnd & \fail & \fail & \fail & \fail \\
        DemonAttack & \mathbf{20} \pm 00 & 99 \pm 01 & \mathbf{98} \pm 01 & 99 \pm 02 \\
        Hero & \mathbf{48} \pm 04 & 96 \pm 03 & \mathbf{86} \pm 08 & 96 \pm 04 \\
        IceHockey & \mathbf{65} \pm 20 & \fail & \mathbf{91} \pm 08 & \fail \\
        Jamesbond & \mathbf{30} \pm 13 & 68 \pm 06 & \mathbf{59} \pm 20 & 67 \pm 06 \\
        Krull & \mathbf{75} \pm 12 & 99 \pm 01 & \mathbf{35} \pm 21 & 98 \pm 02 \\
        Phoenix & \mathbf{30} \pm 00 & 92 \pm 07 & 97 \pm 00 & \mathbf{92} \pm 07 \\
        Pong & \mathbf{21} \pm 03 & 79 \pm 03 & \mathbf{42} \pm 01 & 78 \pm 03 \\
        Qbert & \mathbf{40} \pm 00 & 100 \pm 00 & \mathbf{84} \pm 04 & 100 \pm 00 \\
        Riverraid & \mathbf{95} \pm 05 & 100 \pm 00 & \mathbf{99} \pm 01 & 100 \pm 00 \\
        RoadRunner & \fail & \fail & \fail & \fail \\
        Seaquest & \mathbf{48} \pm 04 & 94 \pm 04 & 92 \pm 04 & \mathbf{91} \pm 05 \\
        SpaceInvaders & \mathbf{30} \pm 00 & 100 \pm 00 & \mathbf{93} \pm 00 & 100 \pm 00 \\
        StarGunner & \mathbf{40} \pm 00 & 100 \pm 00 & \mathbf{99} \pm 00 & 100 \pm 00 \\
        YarsRevenge & \fail & \fail & \fail & \fail \\
		\bottomrule
    \end{tabularx}
    \normalsize
\end{table*}

We observe that using our ranking method enables a
significant pruning of the policies, while maintaining performance.
To answer {\bf RQ2}, we experimented with larger and more complex
Atari environments. The results demonstrate that our framework is
reasonably scalable, but also that the quality of the ranking is significantly
improved by using a state abstraction.
The results in the larger and more complex Atari environments show the effect 
of using a test suite that is too small: many states are not 
encountered during the computation of the ranking. This means
that $\mathit{rank}[1]$, in which the original policy is 
used in \emph{all} of the states discovered while making the ranking,
does not recover the performance of the original policy. 
Increasing the size of the test
suite would help, but this is not
a scalable solution. Instead, we use better \emph{state abstractions},
which reduce the state space.
In CartPole, this allows us to tackle a continuous domain. 
In the Atari games, even the generic abstraction we use in all the games is
sometimes not enough
(``\fail'' in Tab.~\ref{tab:pruning}).

To show the potential utility of specialised abstractions, we create one 
for \textit{Breakout} in which we extract the coordinates of the ball 
and paddle. The results obtained with this abstraction
are given in Tab.~\ref{tab:pruning} in the row labelled ``Breakout (abs)''.
While the new abstraction does worse in 
terms of states pruned within the policy, it allows us to reach 90\% 
of the policy's original performance with 13\% fewer steps in which we 
use $\pi$ over the default action.

\subsection{Discussion}
\label{sec:discussion}

\paragraph{SBFL ranking for better understanding the RL policy}
Any strong claim about the ranking's application to interpretability requires a user study, which is out of scope of this paper.
However, we can look to existing research looking at the usefulness of SBFL. While some studies suggest that the users typically do not go over the list of possible
causes generated by SBFL linearly (and hence question the usefulness of the ranking)~\cite{PO11}, a recent
large-scale study demonstrates statistically significant and substantial improvements for the users
who use an SBFL tool, and the results hold even for ``mediocre'' SBFL tools~\cite{XBLL16}.
Based on this evidence,
we suggest that the ranking can be used to explain policy decisions,
as the ranked list itself would be helpful to identify the most important decisions.
%We can also perform post-processing on the ranked list and highlight
%the highest-ranked decisions.
In addition, the pruned policies that we construct
are simpler than the original policies while achieving a comparable performance, which can make identifying problems 
more straightforward. Examples are 
presented in the CartPole and Minigrid
sections of the website. Finally, in Fig.~\ref{fig:heatmap}, 
we show a heatmap of the scores of each state of a minigrid environment. 
In each grid square, the agent can be facing four directions. 
We show the score based on the tarantula measure
for these directions from blue (lowest) to red (highest). We show this only for
the states visited along a path to the goal.
Our heatmap gives information 
about the general behaviour of the policy. In this case, points at which 
the agent needs to turn are more red (more important) than points where 
the agent is walking in a straight line. To understand why the downward-facing
states in the right-most column are considered important, refer to our 
website for a full heatmap and explanation.

\begin{figure}
    \centering
    \includegraphics[width=0.25\linewidth]{new_imgs/minigrid/minigrid_path_heatmap.png}
    \caption{Example of a heatmap made based on scores.
        Colour from least to most important are blue, white and red.
        \textbf{(a)}
        Our heatmap based on the Tarantula measure, 
        showing all the states an agent encounters while 
        walking to the goal, including the direction in which 
        the agent was facing. For example, in the top left grid location,
        we show the importance of the state in which the agent is facing 
        right, and the state in which it is facing down.}
    \label{fig:heatmap}
\end{figure}

\paragraph{A Different Default Action}
Not all environments have an obvious default action.
In this case, a straightforward choice is to set the default action to ``take a random action''. 
We measured the effect of this choice by running the same experiments with the changed
default action, and detailed results are available in \ifArxiv{Appendix~\ref{sec:randact}}. 
The results are similar or slightly worse to the ones obtained with the default action ``repeat the previous action''.
%In general this made the results worse,
%but only slightly. 
In most games, the difference was small ($\leq 10\%$); a few games show a marginal improvement.% and in some results improve marginally.
These results indicate that the choice of a default action has no effect on our conclusions. 

%This difference reflects how, in some games, it can be easier or %harder to replace actions 
%with a random action than the previous one. Whether using a %random action as the default action 
%works is likely to be very context dependent. However, we find %that in situations in which 
%there is no clear alternative, it can be successfully used. 

\paragraph{Good vs.~bad policies}
Finally, we performed some initial work towards using the ranking to understand the 
difference between high and low-performing policies. To this end, we produced
a ranking according to the high-performing policy, and then compared how the two
policies behaved in the highest ranked states. Interestingly, our experiments demonstrate that
the high performing and low performing policies agree on $80\%$ of the actions in the top $10\%$ of states. 
This suggests that the policy training (in CartPole)
first picks the
`low-hanging fruit' by performing well in the most
important states. The difference between a high-performing and a low-performing 
policy is mostly in the 
lower-ranked states. Full results for this experiment are 
available in \ifArxiv{Fig.~\ref{fig:cpolegoodbad} in the Appendix}.

%\subsection{Understanding low-performance policies}
%We now use the ranking of states to compare the high-quality policy used 
%in previous experiments (achieving the maximum 
%possible average reward of $200$)
%and an alternative low-quality policy, which achieves an average reward of $97$
%in the CartPole environment. 
%We rank the states using the Tarantula
%measure in Equation~(\ref{eq:tarantula}), as it is one of the best-performing measures on CartPole.
%Then we compare the decisions made by the high-quality policy with
%those by the low-quality policy.
%Figure~\ref{fig:goodbadpolicy} shows that in the top-ranked states, the policies are 
%more likely to agree; in the top $10\%$ of states, the policies agree on
%$80\%$ of actions, and this lowers quasi-linearly as we include more states.
%This suggests that the low-quality policy has 
%already learned to perform well in the most important 
%states, and the difference between the high-quality and the low-quality 
%policy is down to the fine-tuning behavior in the lower-ranked states.

% \subsection{Comparison to existing work}

% Our results are difficult to compare to any existing work, as we are 
% not aware of any methods with similar goals to our own; to rank the 
% decisions made by a policy according to their importance. However, 
% some comparisons can be made based on the possible applications of 
% our ranking, the most obvious being interpretability. While the 
% user study that would be required to make strong claims is outside
% of the scope of this work, we explore a comparison to provide
% intuition. In Fig.~\ref{fig:heatmap}, we show how a heatmap 
% derived from our ranking differs from a conventional saliency map,
% based on taking the gradient of the policy's decision with respect to the 
% state~\cite{greydanus2017visualizing}. Our heatmap gives information 
% about the general behaviour of the policy. In this case, points at which 
% the agent needs to turn are redder (more important) than points where 
% the agent is walking in a straight line. To understand why the downward-facing
% states in the right-most column are considered important, refer to our 
% website for a full heatmap and explanation.
% On the other hand, the more conventional heatmap only shows information
% about a single decision (in this case, the one made in the initial state). 
% We explore how other methods that create 
% policy-level explanations differ from ours in Section~\ref{sec:related}.

% \begin{wrapfigure}{l}{0.5\linewidth}
%     % \begin{subfigure}[t]{0.5\linewidth}
%         \centering
%         \includegraphics[width=0.5\linewidth]{new_imgs/minigrid/minigrid_path_heatmap.png}
%     %     \caption{}
%     %     \label{fig:our_heatmap}
%     % \end{subfigure}\hfill%
%     % \begin{subfigure}[t]{0.5\linewidth}
%     %     \centering
%     %     \includegraphics[width=0.5\linewidth]{new_imgs/minigrid/conventional_heatmap.png}
%     %     \caption{}
%     %     \label{fig:conv_heatmap}
%     % \end{subfigure}

%     \caption{Example of a heatmap made based on scores.
%         Colour from least to most important are blue, white and red.
%         \textbf{(a)}
%         Our heatmap based on the Tarantula measure, 
%         showing all the states an agent encounters while 
%         walking to the goal, including the direction in which 
%         the agent was facing. For example, in the top left grid location,
%         we show the importance of the state in which the agent is facing 
%         right, and the state in which it is facing down.}
%     \label{fig:heatmap}
% \end{wrapfigure}



==> Ranking Policy Decisions/introduction.tex <==
\section{Introduction}

Reinforcement learning is a powerful 
method for training policies that
complete tasks in complex environments.
The policies produced are optimised to maximise 
the expected reward provided by the environment. While
performance is clearly an important goal, 
the reward typically does not capture the 
entire range of our preferences. By focusing solely on 
performance, we risk overlooking the demand for
models that are easier to analyse, 
predict and interpret~\cite{lewis2021deep}.
Our hypothesis is that many trained policies
are \emph{needlessly complex}, i.e., that there
exist alternative policies that
perform just as well or nearly as well
but that are significantly simpler.
This tension between performance and simplicity 
is central to the field of explainable AI (XAI), and 
machine learning as a whole~\cite{gunning2019darpa};
our method aims to help by highlighting the most important 
parts of a policy.

The starting point for our definition of ``simplicity'' is
the assumption that there exists a way to make a ``simple choice'',
that is, there is a %meaningful 
simple default action
for the environment. We argue that this is the case
for many environments in which RL is applied: for example,
``repeat previous action'' is a straightforward default action
for navigation tasks. 

The key contribution of this paper is a novel method for
\emph{ranking policy decisions} according to their importance
relative to some goal. We argue that the ranked list of decisions
is already helpful in explaining how the policy operates.
We evaluate our ranking method by
using the ranking to simplify policies without compromising performance,
%The key contribution of this paper is a novel method for
%simplifying policies without compromising performance,
hence addressing one of the main hurdles for wide adoption
of deep RL: the high complexity of trained policies.
%
%We then define the \emph{complexity} of
%an execution to be the fraction of decisions that differ
%from the default, and we argue that the decisions that
%are truly important are those that deviate.
%This natural tension between performance and simplicity 
%is central to the field of explainable AI (XAI), and 
%machine learning as a whole~\cite{gunning2019darpa}.

We produce a ranking
by scoring the states a policy visits. The rank reflects
the impact that replacing the policy's chosen action by
the default action has on a user-selected binary outcome, such as
``obtain more than X reward''.
It is intractable to compute this ranking precisely, owing to the
high complexity and the stochasticity of the environment and the policy, 
complex causal interactions between actions and their outcomes,
and the sheer size of the problem. 
%
%There are many challenges to computing this ranking: the 
%stochasticity of the environment and policy; the complex 
%causal interactions between actions and the outcomes; 
%the sheer number of states being visited. Some states may only be important 
%if considered in groups, and others' importance may or may 
%not depend on subsequent actions. A successful ranking 
%should take all of these into account, and the number of 
%considerations makes a na\"ive approach to ranking the states intractable.
Our work uses \emph{spectrum-based fault localisation}
(SBFL) techniques~\cite{naish2011model,wong2016survey}, borrowed from the software
testing domain, to compute an approximation of the ranking of policy decisions.
%
%Our proposal is to apply spectrum-based fault localisation
%(SBFL)~\cite{naish2011model} to make the problem of ranking
%policy decisions tractable. 
SBFL is an established technique
in program testing for ranking the parts of a program
source code text that are most likely to contain the
root cause of a bug. This ranking is computed by recording
the executions of a user-provided test suite. SBFL distinguishes
passing and failing executions; failing executions are those
that exhibit the bug. Intuitively, a program location is
more likely to be the root cause of the bug if it is visited
in failing executions but less (or not at all) in passing ones.
%SBFL is designed to deal with complex causal relationships
%between entities like those found in program code.
SBFL is a lightweight technique and its rankings are 
highly correlated with the 
location of the root cause of the bug~\cite{wong2016survey}.
We argue that SBFL is also a good fit for analysing complex RL policies.
%We argue therefore that it is a good fit for policies
%with complex causal relationships between decisions.

% SBFL is known to require a balanced test suite \cite{wong2016survey}; that is, the number
% of passing and failing tests should be roughly the same. Conversely,
% a suite of tests that all fail or all pass delivers no result.
% This presents a challenge when applying SBFL to policies
% trained using RL. It is common that a well-trained policy
% succeeds most of the time. Furthermore,
% a well-trained policy may yield a set of executions that
% only exercises a small fraction of the state space, which
% means that no information is gained about (hypothetical)
% decisions in other states. Our algorithm therefore enriches the test suite using
% \emph{mutant executions}, which are runs in which random
% decisions are replaced by the default. We adjust the mutation
% rate to obtain a balanced ratio of failing and passing runs.

Our method applies to RL policies in a black-box manner, and requires
no assumptions about the policy's training or representation. We evaluate
the quality of the ranking of the decisions by the proxy of creating new,
simpler policies (we call them ``pruned policies'') without retraining,
and then calculate the
reward achieved by these policies. Experiments with agents
for MiniGrid (a~more complex version of gridworlds)~\cite{gym_minigrid},
CartPole~\cite{DBLP:journals/corr/BrockmanCPSSTZ16} and
a number of Atari games~\cite{DBLP:journals/corr/BrockmanCPSSTZ16}
demonstrate that pruned policies maintain high performance (similar or
only slightly worse than that of the original policy) when
taking the default action in the majority of the states (often $90\%$
of the states).
%that it is possible to maintain high performance while
%taking the default action in most states. 
As pruned policies are much easier to understand than the original policies,
we consider this an important step towards explainable RL. 
% In addition,
% replacing an original policy with a pruned one can save power by limiting the
% number of decisions actively taken by the agent. 
Pruning a given policy does not require re-training, and hence,
our procedure is relatively lightweight.
Furthermore,
the ranking of states by itself provides important insight into the importance
of particular decisions for the performance of the policy overall.

%Perhaps counter-intuitively,
%we observe that decisions made in states visited most frequently
%in our set of benchmarks are not necessarily the most important ones.

The code for reproducing our experiments is available on GitHub\footnote{\url{https://github.com/hadrien-pouget/Ranking-Policy-Decisions}. Experiments done at commit
c972414}, 
and further examples are provided on the project
website\footnote{\url{https://www.cprover.org/deepcover/neurips2021/}}.

% https://sites.google.com/view/ranking-policy-decisions/

\begin{figure}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width=0.49\linewidth]{new_imgs/cartpole/freqVis.png}\hfill%
        % \includegraphics[width=0.3\linewidth]{new_imgs/cartpole/ochiai_center.png}\hfill%
        \includegraphics[width=0.49\linewidth]{new_imgs/cartpole/ochiai_outside.png}
        \caption{}
        \label{fig:vis_1}
    \end{subfigure}\hfill%
    \begin{subfigure}[t]{0.52\linewidth}
        \centering
        \hfill
        \includegraphics[width=0.47\linewidth]{new_imgs/minigrid/not_lazy_trace.png}\hfill%
        \includegraphics[width=0.47\linewidth]{new_imgs/minigrid/lazy_trace.png}\hfill
        \caption{}
        \label{fig:vis_2}
    \end{subfigure}
    \caption{\textbf{(a)} CartPole, in a state where the cart and pole are moving rapidly.
        The heatmap represents 
        the frequency of appearance of the possible pole 
        angles (left) and the importance scores following SBFL (right). While
        it is more frequent for the pole to be 
        centred, SBFL successfully identifies that the policy's decisions are 
        more important when the pole is close to falling.
        \textbf{(b)} MiniGrid. Traces of executions with the original policy (left) and a \emph{pruned policy} (right). States in which 
        we take the default action are in blue. Both policies succeed, but pruning unimportant actions simplifies the policy.}
\end{figure}


==> Ranking Policy Decisions/related.tex <==
\section{Related work}
\label{sec:related}

%Our method complements 
%existing explainability methods
%such as saliency maps \cite{greydanus2017visualizing,schk2020}, attention models 
%\cite{DBLP:conf/nips/MottZCWR19,DBLP:journals/corr/abs-2003-07069}, 
%or other methods focused on explaining single actions 
%\cite{DBLP:conf/aies/EhsanHCR18,DBLP:journals/corr/abs-1807-08706},
%by highlighting the decisions that are the ones most worth explaining.

There is a significant body of work on identifying the important parts of
trained algorithms, but to the best of our knowledge none suggested to rank
the states as we do.  Prioritised experience
replay~\cite{DBLP:journals/corr/SchaulQAS15} looks for the most important
\emph{transitions} for training.  Saliency
maps~\cite{greydanus2017visualizing,wang2015dueling,zahavy2016graying}
identify the parts of the state that most influence influence
the agent’s decision. \citet{schk2020} have previously applied SBFL  to visual feature
importance for input images given to image classifiers.
Other attempts include identifying the important parts of the \textit{representation} of
the policy by looking at the parameters of a trained model and pruning it to reduce
its size~\cite{livne2020pops}.  None of these methods attempt to understand
what the important decisions of the policy as a whole are.

Much of the recent work focuses on making deep learning models more
interpretable~\cite{lime,shap,schk2020}.  Many
approaches~\cite{greydanus2017visualizing,wang2015dueling,zahavy2016graying}
to explaining deep reinforcement learning methods explain the decision made in a single
state, without the context of the past or the future behaviour. 
\citet{iyer2018transparency} explain a single decision via an object-level
saliency map by leveraging the pixel-level explanation and object
detection. 
As these methods focus on single decisions, the explanation is
typically not sufficient to understand the overall decision-making of the trained agent.

Other work has also attempted to explain entire policies, rather than individual decisions. 
\citet{ehsan2018rationalization} produce natural language explanations for state-action pairs,
based on a human-provided corpus of explanations. \citet{topin2019generation} 
create a Markov chain which acts as an 
abstraction of the policy, making it easier to reason about the policy. They 
create the Markov chain by grouping states into abstract states based 
on how similarly the policy acts in those states; our method is 
substantially different in that it ranks states based on importance, 
rather than grouping similar states. While our method allows for the 
use of abstract states, it is not always necessary, and we are not 
contributing any specific abstraction function.
%The graphs are also only shown for relatively simply environments, and not tested on environments as complex as Atari games.
Similarly, \citet{DBLP:conf/aips/SreedharanSK20} propose a 
method for creating a temporal abstraction of a policy by using 
bottleneck `landmarks' in the policy's executions. A robot's behaviour
can be explained using operator-specified
``important program state variables'' and ``important functions'' \cite{hayes2017improving}.  
We find that the policy-wide decision ranking in this paper is an easier and more
general method for understanding the policy.
For more work in this vein, we encourage the reader to consult the overview from
\citet{DBLP:conf/ijcai/ChakrabortiSK20} of the 
rapidly growing field of Explainable AI Planning (XAIP).

There have been attempts to make more interpretable models, either from
scratch~\cite{hein2018interpretable}, or by approximating a trained neural
network~\cite{verma2018programmatically}.  In the latter case, our method
may be useful for determining in which states the approximation must be most
accurate.

% Given the success of RL in applications that include safety-critical scenarios,
% reducing the complexity of trained policies (while preserving the performance) becomes useful
% for checking for the consistency with specifications or interpreting the policies.
% Imitation learning~\cite{schaal1999imitation} reduces the complexity of reinforcement learning algorithms
% by using expert demonstrations for certain behaviors.
% Recent work on RL with programmatic policies~\cite{verma2018programmatically} applies syntactic
% restrictions to prune undesired policies. Their objectives are similar to our paper's
% wrt.~structural simplicity of a policy,
% although the techniques are very different. Following the line of work for reducing
% the size of the trained model, \cite{livne2020pops} trains policies represented
% as deep neural networks (DNNs) with the goal of obtaining a small DNN.

% Many recent works make DNNs more interpretable~\cite{lime,shap,schk2020}.
% %The majority of the existing work in explaining deep learning models explains
% %only a single decision in terms of input features~\cite{lime,shap,schk2020}.
% In \cite{schk2020}, SBFL is applied to visual feature
% attributions on input images given to feed-forward DNN classifiers. Similarly,
% many existing approaches~\cite{greydanus2017visualizing,wang2015dueling,zahavy2016graying}
% to explaining RL
% agents share techniques used for explaining deep neural network predictions, and they focus on generating saliency
% maps to understand the magnitude of policy changes as a function of a perturbation of the input.
% As a result, the explanation is not sufficient for the stakeholder to gain trust in the overall decision making in the RL system.
% In \cite{iyer2018transparency}, a single decision in the RL policy is explained via an object-level saliency map by leveraging the pixel level explanation and the object detection. In \cite{ehsan2018rationalization}, natural language explanations are created for each action the RL agent performs. These explanations are based on the human-provided corpus of explanations. 
% In \cite{topin2019generation}, the approach starts with creating a full-policy abstraction,
% so that individual decisions can be explained in the context of expected future transitions.
% Interpretable RL policies are studied in \cite{hein2018interpretable}, who rely on the
% intrepretable RL modelling.
% \cite{khan2009minimal}, given a known model of the environment, creates explanations
% by populating a set of pre-defined templates. The robot's behavior in \cite{hayes2017improving} is explained using operator-specified
% ``important program state variables'' and ``important functions''.
% In contrast, policy-wise decision ranking in this paper is an easier and more general method for understanding the RL policy making.

%\paragraph{Robustness of RL}
%Our work is also innovative for improving the robustness of RL policies: given a policy $\pi$,
%we generate a lazier version of it that is more robust, based on $\pi$'s decision ranking.
%This is a different perspective from existing research.
%In terms of robustness, in \cite{rajeswaran2016epopt},
%a robust policy is learned by sampling the worst
%case trajectories from a class of parametrized models.
%The idea of robust adversarial reinforcement learning is proposed in \cite{pinto2017robust},
%where an agent is trained to operate in the presence of a destabilizing adversary that applies disturbance forces to the system.
%The jointly trained adversary is reinforced to learn an optimal destabilization policy.
%In \cite{mankowitz2019robust}, environment perturbations are incorporated into the RL model for training the RL agent.

%\paragraph{Software engineering for robust deep learning}
%Software testing has been the primary approach for increasing stakeholders' confidence on software product and services.
%Coverage-guided testing has been recently applied to testing learning models. especially against adversarial
%behaviours \cite{}. \cite{} discover that adversarial testing problem can be formulated in the way
%of differential software testing. \cite{} apply spectrum-based fault localization in a white-box manner and to localizing
%important neurons in a deep neural network that are for its adversarial output. None of above mentioned work considers the RL
%context.


==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
